Could the Universe have an Exotic Topology?

A recent article uncovered a surprising dynamical mechanism at work within the (vacuum) Einstein `flow' that strongly suggests that many closed 3-manifolds that do not admit a locally homogeneous and isotropic metric \textit{at all} will nevertheless evolve, under Einsteinian evolution, in such a way as to be \textit{asymptotically} compatible with the observed, approximate, spatial homogeneity and isotropy of the universe \cite{Moncrief:2015}. Since this previous article, however, ignored the potential influence of \textit{dark-energy} and its correspondent accelerated expansion upon the conclusions drawn, we analyze herein the modifications to the foregoing argument necessitated by the inclusion of a \textit{positive} cosmological constant --- the simplest viable model for dark energy.

==> sec-hamiltonian.tex <==
\section{Hamiltonian Reduction}%section 3; section 4 as of Jan. 15, 2019
\label{sec:Hamiltonian}

Hamiltonian reduction of Einstein's equations can be globally formulated most readily for manifolds of negative Yamabe type and for spacetimes that admit foliations by Cauchy hypersurfaces of constant mean curvature. A constant mean curvature (or CMC for brevity) hypersurface might be described intuitively as one with a (spatially) uniform `Hubble constant'. This assumption allows (not only in vacuum but also with suitable matter sources) a very convenient decoupling and resolution of the Einstein constraint equations through an application of the well-known conformal method \cite{present,Choquet-Bruhat:2009,Bartnik:2004}.  The inclusion of specific sources for the construction of more realistic cosmological models is hampered by the difficulty in constructing adequate models for fluid matter that evolve without singularity in the inhomogeneous situations of interest here. For simplicity of presentation we shall therefore sidestep those issues and sketch only the reduction procedure restricted to the case of vacuum spacetimes.

Any element of $\mathfrak{J}  (M)$ is a conformal class that can be concretely represented by a specific metric $\gamma$ having scalar curvature $R(\gamma) = -1$. To avoid over-counting though one should restrict the choice of such metrics to a slice for the action of $\mathcal{D}_0 (M)$ on  $\mathcal{M}_{-1} (M)$ or, in physicists' language, one should fix the spatial gauge. The choice of such a slice can be thought of geometrically as the choice of a (possibly only local) `coordinate chart' for  the reduced configuration space $\mathfrak{J}  (M)$. If the mean curvature is designated by a (spatial) constant $\tau$ then, as is well-known, the momentum constraint equation has a general solution, for a fixed value of $\tau$, that is parametrized by the choice of $\gamma$ and by a tensor density $p^{TT}$ that is symmetric, traceless and divergence-free (or `transverse-traceless' in the usual terminology) with respect to  $\gamma$.

A solution of the remaining, Hamiltonian constraint is then determined (for any non-zero value of  $\tau$) by solving the corresponding Lichnerowicz equation for the appropriate conformal factor $\varphi =   \varphi( \tau,  \gamma,  p^{TT})$ that is uniquely and smoothly determined thereby as a functional of its indicated arguments \cite{Fischer:2002}. The variables $\{ \gamma,  p^{TT}\}$, with  $\gamma$ restricted to a slice and  $p^{TT}$ as above, can be viewed as providing a canonical chart for the cotangent bundle, $T^* \mathfrak{J}  (M)$, of the configuration space $\mathfrak{J}  (M)$, which is the natural reduced phase space for the associated (reduced-) Hamiltonian system defined by Einstein's equations in this gauge.

It is not difficult to show that, relative to any time function  $t$ adapted to the CMC slicing (i.e. having CMC level surfaces), the mean curvature  $\tau$ must vary monotonically. We can therefore specify a (CMC) time gauge completely by choosing  $t$ to be a particular monotonic function of  $\tau$. A natural choice to make from the present point of view is given by  $t  =  t(\tau)  = 2/(3 (-\tau)^2)$ since this leads directly to the specific reduced Hamiltonian we wish to discuss. This latter functional is now given by the (dimensionless) expression:
\begin{equation}
H_{\mathrm{reduced}} (\tau , \gamma ,  p^{TT}) = (-\tau)^3 \int_{M} \varphi^6 (\tau , \gamma ,  p^{TT}) d\mu_\gamma
\label{eq:03}
\end{equation}
where $d\mu_\gamma$   is the Riemannian measure on M determined by the conformal metric  $\gamma$ and, in our sign conventions,  $-\tau > 0$ for an expanding universe \cite{Fischer:2002b,Andersson:2011}. Reexpressed in terms of the `physical' spatial metric $g = \varphi^4   \gamma$,  $H_{\mathrm{reduced}}$ is simply the actual spatial volume rescaled (to make it dimensionless) by the cube of  $-\tau$:
\begin{equation}
H_{\mathrm{reduced}} ( \tau,  \gamma,  p^{TT}) = (-\tau)^3 \int_{M} d\mu_g.
\label{eq:04}
\end{equation}
Through it's explicit (especially via  $\varphi( \tau,  \gamma,  p^{TT}))$ dependence on the `time' coordinate function  $t  = 2/(3 (-\tau)^2)$, which has the natural maximal range $(0, \infty)$ --- vanishing at the big bang and blowing up in the limit of infinite expansion --- $H_{\mathrm{reduced}}$ cannot be a conserved quantity in general.\footnote{ Mathematically one would normally formulate the reduced dynamics on a so-called contact manifold  diffeomorphic to $T^* \mathfrak{J}  (M) \times R^+$  but we shall instead adopt the physicists' convention of working with a time dependent Hamiltonian on the symplectic manifold  $T^* \mathfrak{J}  (M)$.\label{note02}} A straightforward calculation, which generalizes as well to other  dimensions and even has a suitably defined, quasi-local analogue \cite{Fischer:2002b}, shows however that $H_{\mathrm{reduced}}$ is strictly \textit{monotonically decreasing} in the direction of cosmological expansion except for a family of continuously self-similar spacetimes \cite{Fischer:2002b,Andersson:2011}, which correspond to its critical points, for which this Hamiltonian is actually constant.

These self-similar solutions exist if and only if M admits an Einstein metric, that is a Riemannian metric $\gamma \in  \mathcal{M}_{-1} (M)$ for which the Ricci tensor $\mathrm{Ric}(\gamma)$ is a (negative) constant multiple of the metric.  In three spatial dimensions the Mostow rigidity theorem excludes all but stand-alone hyperbolizable manifolds (for which the corresponding Einstein metrics are in fact hyperbolic and unique modulo isometries) while in higher dimensions (as well as in $2 + 1$ dimensions) nontrivial families of non-isometric Einstein metrics can arise to determine (finite dimensional) submanifolds of the reduced configuration spaces $\mathfrak{J}  (M) = \mathcal{M}_{-1}  (M) / \mathcal{D}_0 (M)$. When these self-similar solutions do arise (in $n + 1$ dimensions, $n \geq 2$) their corresponding line elements take the form:
\begin{equation}
ds^2 =  -(n /  \tau^2)^2  d\tau^2  +  [(n/(n - 1)) / \tau^2]  \gamma_{i j}  dx^i dx^j
\label{eq:05}
\end{equation}
where here  $\gamma$ is a fixed (time-independent) Einstein metric with Ricci tensor  $\mathrm{Ric}(\gamma) = -\gamma / n$.  We shall refer to such spacetimes as `Lorentz cones' over their corresponding Riemannian Einstein spaces $(M, \gamma)$. In a later section we shall discuss the dynamical stability of such Lorentz cones in the direction of cosmological expansion. In $2 + 1$ and $3 + 1$ dimensions, such vacuum self-similar solutions have vanishing spacetime curvature but in higher dimensions the (moduli) spaces of such solutions can be vastly richer and the corresponding stability problems accordingly more intricate.



==> sec-sigma-constant.tex <==
\section{The $\sigma$ Constant and its Cosmological Significance}%section 4
\label{sec:sigma-Constant}

Since the reduced Hamiltonian is bounded from below (as the rescaled volume of CMC 	
hypersurfaces) and is universally monotonically decaying in the direction of cosmological expansion it is natural to ask what it is decaying towards. The answer is provided by a theorem that characterizes the infimum of $H_{\mathrm{reduced}} (\tau ,\gamma ,  p^{TT})$ (taken, at fixed  $\tau$, over all $T^* \mathfrak{J}  (M)$) in terms of a topological invariant known as the $\sigma$ constant (or Yamabe invariant) of M  \cite{Schoen:1989,Anderson:1997}:
\begin{equation}
\underset{(\gamma,  p^{TT}) \in  T^* \mathfrak{J}  (M)}{\mathrm{inf}}\quad H_{\mathrm{reduced}} (\tau, \gamma,  p^{TT}) = ( n/(n - 1) (-\sigma (M)))^{n/2}.
\label{eq:06}
\end{equation}
The $\sigma$ constant is, in a sense, a natural generalization of the Euler characteristic $\chi(\Sigma_p)$ of a compact surface since, when restricted to two dimensions, its definition leads to:
\begin{equation}
\sigma (\Sigma_p)  =  4 \pi\; \chi(\Sigma_p) =  8  \pi (1 - p).
\label{eq:07}
\end{equation}
More generally, for manifolds of negative Yamabe type in higher dimensions, the precise definition leads to the formula:	
\begin{equation}
\sigma (M)  =   - \left(\underset{\gamma \in  \mathcal{M}_{-1} (M)}{\mathrm{inf}}\quad   \mathrm{vol}(M,\gamma) \right)^{2/n}.
\label{eq:08}
\end{equation}
	
